Homotopy theory of equivariant operads with fixed colors

We build model structures on the category of equivariant simplicial operads with a fixed set of colors, with weak equivalences determined by families of subgroups. In particular, by specifying to the family of graph subgroups (or, more generally, one of the indexing systems of Blumberg-Hill), we obtain model structures on the category of equivariant simplicial operads with a fixed set of colors, with weak equivalences determined by norm map data.

==> labels-OneColor.tex <==
% AllColors-v2 aux file



% TameAndSquare_v2 aux file


